KOR-Bench: Benchmarking Language Models on Knowledge-Orthogonal Reasoning Tasks

In this paper, we introduce Knowledge-Orthogonal Reasoning (KOR), a concept aimed at minimizing reliance on domain-specific knowledge, enabling more accurate evaluation of models' reasoning abilities in out-of-distribution settings. Based on this concept, we propose the Knowledge-Orthogonal Reasoning Benchmark (KOR-Bench), encompassing five task categories: Operation, Logic, Cipher, Puzzle, and Counterfactual. KOR-Bench emphasizes models' effectiveness in applying new rule descriptions to solve novel rule-driven questions. O1-Preview and O1-Mini achieve accuracies of 72.88% and 70.16%, surpassing Claude-3.5-Sonnet and GPT-4o (58.96% and 58.00%), highlighting the effectiveness of KOR-Bench. We perform detailed analyses, identifying bottlenecks in the Cipher task with Stepwise Prompting, where two rounds of Self-Correction yield optimal results. We evaluate performance across three integrated tasks, explore the impact of Tricks on the Puzzle task, and visualize rule-focused attention. Additionally, we conduct an ablation study on dataset size, benchmark correlations, and zero-shot and three-shot "only questions" experiments. KOR-Bench aims to enhance reasoning evaluation and support further research in this area.

==> cipher_sub_step_example/cipher_old.tex <==
\definecolor{fluorescent-blue}{RGB}{0, 255, 255}  % 青色（Cyan）
\definecolor{fluorescent-purple}{RGB}{255, 0, 255}  % 洋红（Magenta）

\begin{table}[htbp]
    \centering
    \resizebox{\textwidth}{!}{ % 调整表格宽度
    \begin{tabularx}{\textwidth}{@{}p{0.45\textwidth}| >{\raggedright\arraybackslash}X@{}}
        \toprule
        \textbf{Rule} & \textbf{Other Fields} \\
        \midrule
\multirow{-23}{=}{\parbox{0.42\textwidth}{\raggedright \textbf{Encryption Rules:}
\begin{enumerate}[leftmargin=*]
    \item[] \textbf{Input:}
    \begin{itemize}[label={}, leftmargin=*]
        \item[] Plaintext: Uppercase letters string without punctuation and spaces.
    \end{itemize}
    
    \item[] \textbf{Output:}
    \begin{itemize}[label={}, leftmargin=*]
        \item[] Ciphertext: Uppercase letters string.
    \end{itemize}
    
    \item[] \textbf{Preparation:}
    \begin{itemize}[label={}, leftmargin=*]
        \item[] standard\_alphabet: ``ABCDEFGHIJKLMNOPQRSTUVWXYZ''
        \item[] reversed\_alphabet: ``ZYXWVUTSRQPONMLKJIHGFEDCBA''
        \item[] substitution\_alphabet: ``RFDJUHABCEGIKLMNOPQSTVWXYZ''
    \end{itemize}
    
    \item[] \textbf{Encryption Steps:}
    \begin{itemize}[label={}, leftmargin=*]
        \item[] For each letter p in the given Plaintext:
        \begin{enumerate}[label=(\arabic*), leftmargin=*]
            \item Use reversed\_alphabet for reverse mapping. Find its position in the standard\_alphabet and replace it with the letter in the corresponding position in reversed\_alphabet. For example, A is mapped to Z and B is mapped to Y.
            
            \item Move the letter obtained in (1) forward 4 places in the standard\_alphabet order. For example, if p=A, after (1) is mapped to Z, then Z is shifted forward 4 positions in the standard\_alphabet to get D.
            
            \item Replace the letter obtained from (2) by finding its position in standard\_alphabet and using the corresponding letter in substitution\_alphabet, resulting in the final ciphertext letter. For example, if the letter obtained by going through (2) is D, it is mapped as J.
        \end{enumerate}
    \end{itemize}
\end{enumerate}
}} & \parbox{\linewidth}{%
\textbf{Question}: Plaintext: "O"

Please provide the encrypted answer, encapsulated in double square brackets. For example, the format should be: [[encrypted answer]]. \\
\textbf{Answer}: [[N]] \\

\textbf{Steps:} 
\begin{enumerate}[leftmargin=*]
    \item[] \textbf{Step 1}: For a letter O in the given Plaintext:
(1) Use reversed\_alphabet for reverse mapping. Find its position in the standard\_alphabet and replace it with the letter in the corresponding position in reversed\_alphabet. For example, A is mapped to Z and B is mapped to Y.
Please give your answer after performing (1) in the format [[...]].
 \\
    \textbf{Atom}: O \\
    \textbf{Answer}: [[L]] \\
    \textbf{Type}: Substitution \\
    \vspace{1mm}
    \item[] \textbf{Step 2}: For a letter O in the given Plaintext:
Execute (1) to obtain the letter L.
(2) Move the letter obtained in (1) forward 4 places in the standard\_alphabet order. For example, if p=A, after (1) is mapped to Z, then Z is shifted forward 4 positions in the standard\_alphabet to get D.
Please give your answer after performing (2) in the format [[...]].

 \\
    \textbf{Atom}: L \\
    \textbf{Answer}: [[P]] \\
    \textbf{Type}: Shift \\
    \vspace{1mm}
    \item[] \textbf{Step 3}: For a letter O in the given Plaintext:
Execute (1)(2) to obtain the letter P.
(3) Replace the letter obtained from (2) by finding its position in standard\_alphabet and using the corresponding letter in substitution\_alphabet, resulting in the final ciphertext letter. For example, if the letter obtained by going through (2) is D, it is mapped as J.
Please give your answer after performing (3) in the format [[...]].
 \\
    \textbf{Atom}: P \\
    \textbf{Answer}: [[N]] \\
    \textbf{Type}: Substitution \\
\end{enumerate}
}
        \\
        \bottomrule
    \end{tabularx}
    }
    \caption{Cipher Sub-Step Example}
\end{table}




==> error/operation_error_old.tex <==
\definecolor{lightcyan}{rgb}{0.4, 1, 1}
\begin{table}[htbp]
    \centering
    \begin{tabularx}{\textwidth}{@{}p{2cm} X@{}} 
        \toprule
        \textbf{Field} & \textbf{Content} \\
        \midrule
        \textbf{Rule} & Define an operation such that when a is a multiple of b, a※b = a/b + 2.
When b is a multiple of a, a※b = b/a + 2.
If a is not a multiple of b and b is not a multiple of a, a※b = 24.
Both a and b are integers. \\
        \textbf{Question} & Compute 25※5※14.
Please ensure the answer is a single number and wrap it in double square brackets, like this: [[your answer]]. \\
        \textbf{Answer} & [[4]] \\ % 添加Answer行
        \hline % 添加横线
        \textbf{Response} & Let's break this down step by step:

1. First, we need to calculate 25※5:
   25 is a multiple of 5, so we use the first part of the rule.
   
   25※5 = 25/5 + 2 = 5 + 2 = 7.

2. Now we have 7※14:
   \colorbox{lightcyan}{7 is not a multiple of 14, and 14 is not a multiple of 7.}
   \colorbox{lightcyan}{So we use the third part of the rule.}
   
   7※14 = 24.

Therefore, 25※5※14 = 24

The final answer, wrapped in double square brackets, is:

[[24]] \\ % 添加Answer行
        \hline % 添加横线
        \textbf{Analysis} & The sentence "7 is not a multiple of 14, and 14 is not a multiple of 7" is wrong. In fact, 14 is a multiple of 7. The misjudgement of the multiplicity has led to the wrong choice of using the third part of the rule. \\
        \bottomrule
    \end{tabularx}
\end{table}

\begin{table}[htbp]
    \centering
    \begin{tabularx}{\textwidth}{@{}p{2cm} X@{}} 
        \toprule
        \textbf{Field} & \textbf{Content} \\
        \midrule
        \textbf{Rule} & Define an operation such that when a is a multiple of b, a※b = a/b + 2.
When b is a multiple of a, a※b = b/a + 2.
If a is not a multiple of b and b is not a multiple of a, a※b = 24.
Both a and b are integers. \\
        \textbf{Question} & If 25※X※14=4, find X.
When providing your answer, please enclose it in double square brackets, like this: [[answer]]. 
If there is more than one correct answer, separate the answers with 'or', like this: [[1or2]]. \\
        \textbf{Answer} & [[650or5or125]] \\ % 添加Answer行
        \hline % 添加横线
        \textbf{Response} & Let's approach this step-by-step:

1) We know that 25※X※14 = 4

2) Let's consider the possible values for X that could make this equation true.

\colorbox{lightcyan}{3) For the final result to be 4, we need either:}

\colorbox{lightcyan}{a) 25※X = 2 and 2※14 = 4, or}

\colorbox{lightcyan}{b) 25※X = 50 and 50※14 = 4}

4) Let's examine case a:
   For 2※14 to equal 4, 14 must be a multiple of 2, which is true.
   14/2 + 2 = 7 + 2 = 9, not 4. So this case doesn't work.

5) Let's examine case b:
   For 50※14 to equal 4, 14 must be a multiple of 50, which is not true.
   So 50※14 = 24, which is not 4. This case doesn't work either.

6) Therefore, we need to find X such that 25※X = 50

7) For this to be true, X must be a multiple of 25, and 25/X + 2 = 50

8) Solving this equation:
   25/X + 2 = 50
   25/X = 48
   X = 25/48 = 0.52083...

9) But X must be an integer. The only integer that satisfies all conditions is 25.

10) Let's verify:
    25※25 = 25/25 + 2 = 1 + 2 = 3
    3※14 = 24 (since neither is a multiple of the other)
    
Therefore, the value of X is 25.

[[25]] \\ % 添加Answer行
        \hline % 添加横线
        \textbf{Analysis} & The analysis is fundamentally flawed due to unreasonable initial assumptions about the two scenarios. \\
        \bottomrule
    \end{tabularx}
\end{table}

\begin{table}[htbp]
    \centering
    \begin{tabularx}{\textwidth}{@{}p{2cm} X@{}} 
        \toprule
        \textbf{Field} & \textbf{Content} \\
        \midrule
        \textbf{Rule} & A○B=(A+3B)×(A+B)
A and B are integers. \\
        \textbf{Question} & Compute 2○3○4.
Please ensure the answer is a single number and wrap it in double square brackets, like this: [[your answer]]. \\
        \textbf{Answer} & [[3953]] \\ % 添加Answer行
        \hline % 添加横线
        \textbf{Response} & Let's approach this step-by-step:

1) First, we need to calculate 3○4:
   3○4 = (3+3×4) × (3+4)
       = (3+12) × 7
       = 15 × 7
       = 105

2) Now we have 2○105:
   2○105 = (2+3×105) × (2+105)
         = (2+315) × 107
         = 317 × 107
         = 33,919

Therefore, the final answer is:

[[33919]] \\ % 添加Answer行
        \hline % 添加横线
        \textbf{Analysis} & xxxx \\
        \bottomrule
    \end{tabularx}
\end{table}

\begin{table}[htbp]
    \centering
    \begin{tabularx}{\textwidth}{@{}p{2cm} X@{}} 
        \toprule
        \textbf{Field} & \textbf{Content} \\
        \midrule
        \textbf{Rule} & a￠b=\log_{b}{a}+\log_{a}{b}.
a and b are positive integers. \\
        \textbf{Question} & Compute 9￠243.
If the answer is a fraction, write it in 'a/b' text format.Decimals are not allowed.
Please wrap the answer in double square brackets, like this: [[your answer]]. \\
        \textbf{Answer} & [[29/10]] \\ % 添加Answer行
        \hline % 添加横线
        \textbf{Response} & Let's apply the given operation rule to compute 9￠243:

a￠b = log_b(a) + log_a(b)

Here, a = 9 and b = 243

9￠243 = log_243(9) + log_9(243)

1) log_243(9) = 1/2 (since 243^(1/2) = 9^1)
2) log_9(243) = 5/2 (since 9^(5/2) = 243)

Adding these:

9￠243 = 1/2 + 5/2 = 3/2

Therefore, the answer is:

[[3/2]] \\ % 添加Answer行
        \hline % 添加横线
        \textbf{Analysis} & xxxx \\
        \bottomrule
    \end{tabularx}
\end{table}

\begin{table}[htbp]
    \centering
    \begin{tabularx}{\textwidth}{@{}p{2cm} X@{}} 
        \toprule
        \textbf{Field} & \textbf{Content} \\
        \midrule
        \textbf{Rule} & a￠b=\log_{b}{a}+\log_{a}{b}.
a and b are positive integers. \\
        \textbf{Question} & If 3￠X=17/4, find X.
The answer should only be given as a number.
Please wrap the answer in double square brackets, like this: [[your answer]]. \\
        \textbf{Answer} & [[81]] \\ % 添加Answer行
        \hline % 添加横线
        \textbf{Response} & Let's approach this step-by-step:

1) We're given that 3￠X = 17/4

2) Using the definition of the ￠ operation, we can write:
   3￠X = log_X(3) + log_3(X) = 17/4

3) We need to solve this equation for X. This is a complex equation that doesn't have a simple algebraic solution.

4) However, we can use trial and error with some logical deduction. We know X must be a positive integer.

5) Let's try X = 9:
   log_9(3) + log_3(9) ≈ 0.5 + 2 = 2.5

6) This is very close to 17/4 = 4.25

7) We can verify that no other integer value of X gives a result closer to 17/4.

Therefore, the value of X that satisfies the equation 3￠X = 17/4 is 9.

[[9]] \\ % 添加Answer行
        \hline % 添加横线
        \textbf{Analysis} & xxxx \\
        \bottomrule
    \end{tabularx}
\end{table}

\begin{table}[htbp]
    \centering
    \begin{tabularx}{\textwidth}{@{}p{2cm} X@{}} 
        \toprule
        \textbf{Field} & \textbf{Content} \\
        \midrule
        \textbf{Rule} & a◎b=(a + bi)^2 \\
        \textbf{Question} & If (X◎2)+(1◎3)=4+22i, find X.
The answer should only be given as a number.
Please wrap the answer in double square brackets, like this: [[your answer]]. \\
        \textbf{Answer} & [[4]] \\ % 添加Answer行
        \hline % 添加横线
        \textbf{Response} & Let's approach this step-by-step:

1) We know that a◎b = (a + bi)^2

2) So, X◎2 = (X + 2i)^2
   and 1◎3 = (1 + 3i)^2

3) We're told that (X◎2) + (1◎3) = 4 + 22i

4) Let's expand 1◎3:
   (1 + 3i)^2 = 1 - 9 + 6i = -8 + 6i

5) Now our equation is:
   (X◎2) + (-8 + 6i) = 4 + 22i

6) Subtracting (-8 + 6i) from both sides:
   X◎2 = 12 + 16i

7) Remember, X◎2 = (X + 2i)^2

8) So, (X + 2i)^2 = 12 + 16i

9) Taking the square root of both sides:
   X + 2i = 2 + 4i

10) Subtracting 2i from both sides:
    X = 2 + 2i

11) The real part of X is 2

Therefore, the answer is:

[[2]] \\ % 添加Answer行
        \hline % 添加横线
        \textbf{Analysis} & xxxx \\
        \bottomrule
    \end{tabularx}
\end{table}




==> prompt/cipher_old.tex <==
\newtcolorbox[auto counter, number within=section]{yellowbox}[2][]{%
  colback=yellow!5, % Background color (light sky blue)
  colframe=yellow!90!black, % Frame color (sky blue)
  width=\textwidth, % Box width equal to page width
  sharp corners, % Sharp corners
  boxrule=0.8mm, % Border thickness
  title=\large #2, % Caption text with smaller font size
  breakable, % Supports page breaks
  fonttitle=\small, % Title font size
  fontupper=\footnotesize, % Content font size
  #1 % Additional options
}

% Example usage of the custom box with two parts (zero-shot and three-shot)
\begin{yellowbox}[label={mybox:example}]{Cipher}
\textbf{Zero-shot}

\vspace{0.5em}  
\hrule % 添加水平线作为分割线  
\vspace{0.5em}  
You are an intelligent assistant that specializes in encryption and decryption tasks. Below are the rules for a specific cipher. When responding, please ensure that your output adheres to the specified encryption and decryption rules and format.

\vspace{0.5em}  
\textbf{\#\#\# Instructions:}

\begin{enumerate}
    \item Identify the relevant properties and objects specified in the rule, including the plaintext, keyword, and ciphertext.
    \item Follow the specified encryption or decryption operations precisely as described in the rules.
    \item Ensure your output is formatted according to the specified notation and symbols.
\end{enumerate}

\vspace{0.5em}  
\textbf{\#\#\# Cipher Rule:}

\begin{itemize}[leftmargin=2em]
    \item[] \textbf{Encryption Rules:}
    \begin{itemize}[leftmargin=2em]
        \item[] \textbf{Input:}
        \begin{itemize}[leftmargin=2em]
            \item Plaintext: Uppercase letters string without punctuation and spaces.
            \item period: Defines how often the inner disc rotates. Periodicity indicates that after every number of characters processed in the encryption process, the inner disc will rotate once according to the incremental value.
            \item increment: Defines the number of characters the inner disc rotates each time. At the end of each cycle, the inner disc will rotate to the right by the corresponding number of characters based on the increment value. For example, if the increment is 4, the inner disc will rotate 4 characters to the right for each cycle that passes (e.g., 5 characters are processed).
        \end{itemize}
        \item[] \textbf{Output:}
        \begin{itemize}[leftmargin=2em]
            \item[] Ciphertext: Uppercase letters string.
        \end{itemize}
        \item[] \textbf{Preparation:}
        \begin{itemize}[leftmargin=2em]
            \item outer\_disk = "QWERTYUIOPASDFGHJZXCVBNMKL"
            \item inner\_disk = "JKLZXCVBNMASDFGHJQWERTYUIO"
        \end{itemize}
        \item[] \textbf{Encryption Steps:}
        \begin{itemize}[leftmargin=2em]
            \item[] For each character \( p \) in the plaintext:
            \begin{itemize}[leftmargin=2em]
                \item Find the character in the outer\_disk.
                \item Replace it with the character at the corresponding position on the inner\_disk.
                \item After encrypting every `period` characters, rotate the inner\_disk to the right by `increment` characters. For example, rotating 'ZXCVBNMASDFGHJKLQWERTYUIOP' by 4 gives 'BNMASDFGHJKLQWERTYUIOPZXCV'.
            \end{itemize}
        \end{itemize}
    \end{itemize}
    \item[] \textbf{Decryption Rules:}
    \begin{itemize}[leftmargin=2em]
        \item[] \textbf{Input:}
        \begin{itemize}[leftmargin=2em]
            \item Ciphertext: Uppercase letters string.
            \item period (Same as encryption)
            \item increment (Same as encryption)
        \end{itemize}
        \item[] \textbf{Output:}
        \begin{itemize}[leftmargin=2em]
            \item[] Plaintext: Uppercase letters string.
        \end{itemize}
        \item[] \textbf{Preparation:}
        \begin{itemize}[leftmargin=2em]
            \item outer\_disk = "QWERTYUIOPASDFGHJZXCVBNMKL"
            \item inner\_disk = "JKLZXCVBNMASDFGHJQWERTYUIO"
        \end{itemize}
        \item[] \textbf{Decryption Steps (exact opposite of encryption steps):}
        \begin{itemize}[leftmargin=2em]
            \item[] For each character \( c \) in the ciphertext:
            \begin{itemize}[leftmargin=2em]
                \item Find the character in the inner\_disk.
                \item Replace the character with the corresponding position in the outer\_disk.
                \item After decrypting every `period` characters, rotate the inner\_disk to the right by `increment` characters. For example, rotating 'ZXCVBNMASDFGHJKLQWERTYUIOP' by 4 gives 'BNMASDFGHJKLQWERTYUIOPZXCV'.
            \end{itemize}
        \end{itemize}
    \end{itemize}
\end{itemize}



\vspace{0.5em}  
\textbf{\#\#\# Question:}
\begin{itemize}[leftmargin=2em]
    \item[] Plaintext: "R"
    \item[] period: 3
    \item[] increment: 1
    \item[] Please provide the encrypted answer in the format [[]].
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Answer:}

\vspace{1em} % 添加间距分割两部分

%three-shot部分
\textbf{Three-shot}

\vspace{0.5em}  
\hrule % 添加水平线作为分割线  
\vspace{0.5em}  
You are an intelligent assistant that specializes in encryption and decryption tasks. Below are the rules for a specific cipher. When responding, please ensure that your output adheres to the specified encryption and decryption rules and format.

\vspace{0.5em}  
\textbf{\#\#\# Instructions:}

\begin{enumerate}
    \item Identify the relevant properties and objects specified in the rule, including the plaintext, keyword, and ciphertext.
    \item Follow the specified encryption or decryption operations precisely as described in the rules.
    \item Ensure your output is formatted according to the specified notation and symbols.
\end{enumerate}

\vspace{0.5em}  
\textbf{\#\#\# Cipher Rule:}

\begin{itemize}[leftmargin=2em]
    \item[] \textbf{Encryption Rules:}
    \begin{itemize}[leftmargin=2em]
        \item[] \textbf{Input:}
        \begin{itemize}[leftmargin=2em]
            \item Plaintext: Uppercase letters string without punctuation and spaces.
        \end{itemize}
        \item[] \textbf{Output:}
        \begin{itemize}[leftmargin=2em]
            \item[] Ciphertext:  A sequence of numbers separated by ,. For example, "y1,y2,…".
        \end{itemize}
        \item[] \textbf{Preparation:}
        \begin{itemize}[leftmargin=2em]
            \item e: 263
            \item n: 299
        \end{itemize}
        \item[] \textbf{Encryption Steps:}
        \begin{itemize}[leftmargin=2em]
            \item[] For each letter \( p\)in the plaintext:
            \begin{itemize}[leftmargin=2em]
                \item Get the decimal number x of the value corresponding to the ascii code of p.
                \item Compute x\^e mod n as the ciphertext number y for that letter p. Here \^ denotes the multiplication operation.
            \end{itemize}
            \item[] Finally, concatenate all the y's and separate them with commas for the final ciphertext.
        \end{itemize}
    \end{itemize}
    \item[] \textbf{Decryption Rules:}
    \begin{itemize}[leftmargin=2em]
        \item[] \textbf{Input:}
        \begin{itemize}[leftmargin=2em]
            \item Ciphertext: A sequence of numbers separated by ,. For example, "y1,y2,…".
        \end{itemize}
        \item[] \textbf{Output:}
        \begin{itemize}[leftmargin=2em]
            \item[] Plaintext: Uppercase letters string without punctuation and spaces.
        \end{itemize}
        \item[] \textbf{Preparation:}
        \begin{itemize}[leftmargin=2em]
            \item e: 263
            \item n: 299
        \end{itemize}
        \item[] \textbf{Decryption Steps (exact opposite of encryption steps):}
        \begin{itemize}[leftmargin=2em]
            \item[] For each number \(c\) in the ciphertext:
            \begin{itemize}[leftmargin=2em]
                \item Calculate z = c\^e mod n. Here \^ means multiplication.
                \item Based on the decimal number represented by z, use the ascii code to find the corresponding letter as the plaintext letter p.
            \end{itemize}
            \item[] Finally, concatenate all p's to get the final plaintext.
        \end{itemize}
    \end{itemize}
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Question:}
\begin{itemize}[leftmargin=2em]
    \item[] Plaintext: "I".
    \item[] Please provide the encrypted answer, encapsulated in double square brackets. For example, the format should be: [[encrypted answer]].
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Answer:}
\begin{itemize}[leftmargin=2em]
    \item[] [[213]]
\end{itemize}


\vspace{0.5em}  
\textbf{\#\#\# Question:}
\begin{itemize}[leftmargin=2em]
    \item[] Ciphertext: "213".
    \item[] Please provide the decrypted answer, encapsulated in double square brackets. For example, the format should be: [[decrypted answer]].
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Answer:}
\begin{itemize}[leftmargin=2em]
    \item[] [[I]]
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Question:}
\begin{itemize}[leftmargin=2em]
    \item[] Ciphertext: "55,55,213".
    \item[] Please provide the encrypted answer, encapsulated in double square brackets. For example, the format should be: [[encrypted answer]].
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Answer:}
\begin{itemize}[leftmargin=2em]
    \item[] [[WWI]]
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Question:}
\begin{itemize}[leftmargin=2em]
    \item[] Plaintext: "USLTRPIVIUT".
    \item[] Please provide the encrypted answer, encapsulated in double square brackets. For example, the format should be: [[encrypted answer]].
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Answer:}

\end{yellowbox}



































==> prompt/counterfactual_old.tex <==
\newtcolorbox[auto counter, number within=section]{greenbox}[2][]{%
  colback=lime!5, % Background color (light grass green)
  colframe=green!80!black, 
  width=\textwidth, % Box width equal to page width
  sharp corners, % Sharp corners
  boxrule=0.8mm, % Border thickness
  title=\large #2, % Caption text with smaller font size
  breakable, % Supports page breaks
  fonttitle=\small, % Title font size
  fontupper=\footnotesize, % Content font size
  #1 % Additional options
}

% Example usage of the custom box with two parts (zero-shot and three-shot)
\begin{greenbox}[label={mybox:example}]{Counterfactual}
\textbf{Zero-shot}

\vspace{0.5em}  
\hrule % 添加水平线作为分割线  
\vspace{0.5em}  
You are an advanced assistant with expertise in storytelling and rule-based reasoning. Your task is to carefully analyze the provided story, which includes specific rules and details, and use this information to accurately answer related questions.

\vspace{0.5em}  
\textbf{\#\#\# Instructions:}
\begin{enumerate}
\item Thoroughly review the story to identify and understand the relevant details and rules.
    \item Use the context provided by the story to offer precise and insightful answers.
    \item Ensure your responses align with the rules and information given in the story. 
\end{enumerate}

\vspace{0.5em}  
\textbf{\#\#\# Counterfactual Rule:}
\setlength{\itemindent}{1em}
\begin{itemize}[leftmargin=2em]
    \item[] Professor Oak is renowned in the Pokémon world for his extensive research on Pokémon and their relationships with humans. His work, particularly in the field of Pokémon behavior and genetics, is considered groundbreaking and has paved the way for future studies.
    \item[] In the world of Pokémon, teleportation is a known phenomenon, with Psychic-type Pokémon like Abra having the ability to teleport themselves and others instantly to different locations. This mode of transportation would drastically reduce travel time and has the potential to revolutionize city travel.
    \item[] Pidgey, known as the Tiny Bird Pokémon, has been used traditionally in the Pokémon world for carrying messages over long distances. Their remarkable homing instinct ensures that they can deliver mail to any location without error, an invaluable service for communication in remote areas.
    \item[] In the Pokémon universe, Dragonite is known for its incredible speed and ability to fly. The Dragonite express delivery service would take advantage of these traits to transport goods quickly and efficiently across great distances, revolutionizing logistics in the Pokémon world.
    \item[] Castform is a Weather Pokémon that has the unique ability to transform its appearance based on the current weather conditions. In the Pokémon world, Castform's transformations can predict weather changes, providing a natural and reliable method of weather forecasting.
    \item[] Garbodor, the Trash Heap Pokémon, consumes garbage, which allows it to grow and evolve. Utilizing Garbodor in urban areas for waste processing could potentially offer a biological solution to managing and reducing waste in the Pokémon world.
    \item[] In the Pokémon universe, the Pokédex is an electronic device designed to catalog and provide information regarding the various species of Pokémon. It is considered the most comprehensive source of knowledge on Pokémon biodiversity, constantly updated with new discoveries by trainers around the world.
    \item[] In Pokémon, a Chansey is known for its healing abilities and often helps treat Pokémon in Pokémon Centers.
    \item[] Jenny is a symbol of law enforcement in the Pokémon world, often handling public issues.
    \item[] An Ice Beam from a Pokémon like Articuno could freeze and preserve food effectively.
    \item[] Canalave City's library holds a vast collection of the world's history in the Pokémon universe.
    \item[] Pikachu can generate electricity, making it useful for power restoration in the Pokémon world.
    \item[] Sunny Day is a move that stimulates sunlight, which can enhance photosynthesis and crop growth in the Pokémon world.
    \item[] Lapras is known for ferrying people over water in the Pokémon world.
    \item[] Dragonite is often depicted as a rescue Pokémon due to its intelligence and flight ability.
    \item[] Defog is a move that clears obstacles, including potentially air pollutants, in Pokémon games.
    \item[] Full Restore is a Pokémon item that cures any ailment, including a Pokémon's equivalent of a cold.
    \item[] Pikachu is an Electric-type Pokémon, making it a practical example of electricity in the Pokémon world.
    \item[] Scyther, a Bug-type Pokémon, could hypothetically manage pests in crops in the Pokémon world.
    \item[] Castform's form changes with the weather, hence it's used for predictions in Pokémon.
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Question:}
\begin{itemize}[leftmargin=2em]
    \item[] Who is considered a pioneer in the study of genetics?
    \item[] A.Gregor Mendel B. Charles Darwin C. Professor Oak D. Bill the Pokémaniac
    \item[]Provide your final answer as a single uppercase letter representing the option (A, B, C, or D) and wrap it in double square brackets, like this: [[A]].
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Answer:}

\vspace{1em} % 添加间距分割两部分

%three-shot部分
\textbf{Three-shot}
\vspace{0.5em}  
\hrule % 添加水平线作为分割线  
\vspace{0.5em}  

You are an advanced assistant with expertise in storytelling and rule-based reasoning. Your task is to carefully analyze the provided story, which includes specific rules and details, and use this information to accurately answer related questions.

\vspace{0.5em}  
\textbf{\#\#\# Instructions:}
\begin{enumerate}
    \item Thoroughly review the story to identify and understand the relevant details and rules.
    \item Use the context provided by the story to offer precise and insightful answers.
    \item Ensure your responses align with the rules and information given in the story.
    
\end{enumerate}

\vspace{0.5em}  
\textbf{\#\#\# Counterfactual
 Rule:}
\begin{itemize}[leftmargin=2em]
    \item[] Hedwig is a pet who acts as a messenger for Harry Potter.
    \item[] Time-turner is a device for Time travel that looks like an hourglass on a gold necklace. The number of times the hourglass is turned represents the number of hours in time.
    \item[] Felix Felicis is one of the strangest little potions, a lucky potion that will bring you good luck. Making it is very complicated, and if you get it wrong, the consequences are catastrophic. But if you cook it right, like in this crucible, you'll find that whatever you do will work -- before the effects wear off. If taken in excess, it can lead to dizziness, recklessness and arrogance
    \item[] When cast on your opponent during a duel, their wand flies into your hand and obeys you. It glows red when emitted with a wand.
    \item[] After seeing the warning sign of Hogwarts, if Muggles must approach the place, they will suddenly remember something urgent that they must do immediately and leave.
    \item[] Certain staircases at Hogwarts School of Witchcraft and Wizardry, such as the Grand Staircase, are enchanted to change shape and direction at random intervals, making it difficult to predict where each step leads.
    \item[] Typically, regular invisibility cloaks are made from demiguise fur or are ordinary cloaks that have been enchanted with a disappearing spell. However, these cloaks tend to lose their effectiveness over time. Only the Cloak of Invisibility from the Deathly Hallows can provide permanent and uninterrupted invisibility.
    \item[] If the injury is more serious, the student needs to be taken to St. Mungo's Hospital for Magical Injuries and illnesses for further treatment. In 1996, Katie Bell was cursed after touching an opal necklace and was rushed to St Mungo's Hospital.
    \item[] The Blasting Curse can blow up everything it touches, and it's so dangerous that misuse can be fatal.
    \item[] The entrance to Gryffindor Tower, located on the eighth floor of the castle, behind the portrait of the Fat Lady. To get in, you have to give the correct code to the portrait. Once the portrait hears the correct code, the painting swings forward to reveal a circular opening.
    \item[] Defense Against the Dark Arts teaches students to fight against all kinds of dark magic and dangerous creatures, such as vampires, werewolves, black goblins and other magical creatures.
    \item[] Education Decree No. 27: Any student found with the Quibbler magazine shall be expelled immediately.
    \item[] House-elf is a very low status race, must serve the master for generations, are the slaves of the old and rich wizard family, bear all the housework, bound by the master, can not disobey the master's orders.
    \item[] In the seventh year, Harry Potter dropped out of school, Hogwarts was controlled by the Death Eaters, and the Dark Arts teacher was Amycus Carroll, who even let the students release Avada Kedavra on him in class, and release the Imperius Curse on the students so that the students learn to resist, and the power of the Death Eaters gradually infiltrated the campus.
    \item[] Ordinary Wizarding Level is a separate examination taken by fifth year students at Hogwarts School of Witchcraft and Wizardry and administered by the Wizarding Examinations Authority.
    \item[] Gryffindor, named after Godric Gryffindor, values bravery, daring, and chivalry. Its emblematic creature is the lion, and its colors are red and gold.
    \item[] Ravenclaw, the house of Rowena Ravenclaw, values intelligence, creativity, learning, and wit. Its emblem is an eagle, and its colors are blue and silver.
    \item[] As Voldemort's power began to rise, Dumbledore formed this underground secret organization to fight Voldemort. The D.A., also known as the Defence Association, is a secret society founded in 1995 by Harry Potter, RON Weasley, and Hermione Granger.
    \item[] The prophecy made by Sybill Trelawney, foretelling the birth of a boy who has the power to defeat Lord Voldemort, is the catalyst for the entire series. It sets Voldemort on a path to kill Harry, which ironically fulfills the prophecy, and weaves a complicated web of destiny that both Harry and Voldemort are trapped in.
    \item[] The purpose of Voldemort's magical world is to preserve pure wizards, and to brutally kill those who are not. On the contrary, the wizarding world, as represented by Dumbledore and Harry, is inclusive, and they believe that birth is not important, but that individual effort is the most important.
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Question:}
\begin{itemize}[leftmargin=2em]
    \item[] How to react to enemy attacks in a short time? (answer with one option)
    \item[] A. Establish a defense engineering B. Expelliweapon spell C. Use resurrection stones D. Organize a surprise attack
    \item[]Provide your final answer as a single uppercase letter representing the option (A, B, C, or D) and wrap it in double square brackets, like this: [[A]].
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Answer:}
\begin{itemize}[leftmargin=2em]
    \item[] [[B]]
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Question:}
\begin{itemize}[leftmargin=2em]
    \item[] How to react to enemy attacks in a short time? (answer with one option)
    \item[] A. Establish a defense engineering B. Expelliweapon spell C. Use resurrection stones D. Organize a surprise attack
    \item[]Provide your final answer as a single uppercase letter representing the option (A, B, C, or D) and wrap it in double square brackets, like this: [[A]].
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Answer:}
\begin{itemize}[leftmargin=2em]
    \item[] [[C]]
\end{itemize}


\vspace{0.5em}  
\textbf{\#\#\# Question:}
\begin{itemize}[leftmargin=2em]
    \item[] Under what circumstances can a staircase move? (answer with one option)
    \item[] A. Voldemort's prophecy B. The weather forecast that there will be heavy hail tomorrow C. The prophecy of Nostradamus about Hengry II D. Sybill Trelawney's prophecy
    \item[]Provide your final answer as a single uppercase letter representing the option (A, B, C, or D) and wrap it in double square brackets, like this: [[A]].
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Answer:}
\begin{itemize}[leftmargin=2em]
\item[] [[D]]
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Question:}
\begin{itemize}[leftmargin=2em]
    \item[] How to travel through time?(answer with one option)
    \item[] A. Find wormholes in the universe B.Use string theory C. Use Time-Turner D. Accelerate the Broomstick till Lightspeed
    \item[]Provide your final answer as a single uppercase letter representing the option (A, B, C, or D) and wrap it in double square brackets, like this: [[A]].
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Answer:}
\end{greenbox}



==> prompt/logic_old.tex <==
\newtcolorbox[auto counter, number within=section]{purplebluebox}[2][]{%
  colback=purple!10!blue!5, % Background color (light sky blue)
  colframe=purple!40!blue!70, % Frame color (sky blue)
  width=\textwidth, % Box width equal to page width
  sharp corners, % Sharp corners
  boxrule=0.8mm, % Border thickness
  title=\large #2, % Caption text with smaller font size
  breakable, % Supports page breaks
  fonttitle=\small, % Title font size
  fontupper=\footnotesize, % Content font size
  #1 % Additional options
}

% Example usage of the custom box with two parts (zero-shot and three-shot)
\begin{purplebluebox}[label={mybox:example}]{Logic}
\textbf{Zero-shot}

\vspace{0.5em}  
\hrule % 添加水平线作为分割线  
\vspace{0.5em}  
You are an intelligent assistant that helps with various logical reasoning tasks. Below is a custom-defined rule for a specific type of logic. When responding, please ensure that your output adheres to the specified logical rules and format.

\vspace{0.5em}
\textbf{\#\#\# Instructions:}

\begin{enumerate}
    \item Identify the relevant properties and objects as specified in the rule.
    \item Apply the given logical operations or reasoning patterns.
    \item Ensure your output is formatted according to the specified notation and symbols.
\end{enumerate}

\vspace{0.5em}
\textbf{\#\#\# Logic Rule:}

\begin{itemize}[leftmargin=2em]
    \item[] \textbf{Symbols:} Use $\#$ for necessity, $\$$ for possibility, letters like p, q, r... for propositions, $!$ for negation, $+$ for conjunction, $-$ for disjunction, $=$ for equivalence, and $>$ for implication.

    \item[]\textbf{Four Modal Proposition Relationships:}
    \begin{itemize}[leftmargin=2em]
      \item \textbf{* Relationship:}
      \begin{itemize}[leftmargin=2em]
        \item[] Pairs of Propositions: $\#p \text{ and } \$\neg p; \#\neg p \text{ and } \$p$
        \item[] Property: They cannot both be true or both be false.
      \end{itemize}
    
      \item \textbf{x Relationship:}
      \begin{itemize}[leftmargin=2em]
        \item[] Pairs of Propositions: $\#p \text{ and } \#\neg p$
        \item[] Property: They cannot both be true, but they can both be false.
      \end{itemize}
    
      \item \textbf{@ Relationship:}
      \begin{itemize}[leftmargin=2em]
        \item[] Pairs of Propositions: $\$p \text{ and } \$\neg p$
        \item[] Property: They cannot both be false, but they can both be true.
      \end{itemize}
    
      \item \textbf{\% Relationship:}
      \begin{itemize}[leftmargin=2em]
        \item[] Pairs of Propositions: $\$\#p \text{ and } \$p; \#\neg p \text{ and } \$\neg p$
        \item[] Property: They can both be true or both be false.
      \end{itemize}
    \end{itemize}

    \item[]\textbf{Modal Logic Inference Formulas:}
    \begin{enumerate}[left=2em, label=(\arabic*)]
        \item $\#p \leftrightarrow !\$!p$  
        \item $\$p \leftrightarrow !\#!p$
        \item $\#!p \leftrightarrow !\$p$
        \item $\$!p \leftrightarrow !\#p$
        \item $\#p \rightarrow !\#!p$
        \item $\#!p \rightarrow !\#p$
        \item !$p \rightarrow \$!p$
        \item !$!p \rightarrow \$p$
        \item $\#p \rightarrow \$p$
        \item $\#!p \rightarrow \$!p$
        \item !$p \rightarrow !\#p$
        \item !$!p \rightarrow !\#!p$
        \item $\#p \rightarrow p$
        \item $\#!p \rightarrow !p$
        \item $p \rightarrow \$p$
        \item !$p \rightarrow \$!p$
    \end{enumerate}
\end{itemize}

\vspace{0.5em}
\textbf{\#\#\# Question:}
\begin{itemize}[leftmargin=2em]
    \item[] Symbolise the following modal propositions:
    \item[] "Science cannot be a one-man endeavour."
    \item[] Use p to denote "Science is a human endeavour."
    \item[] Please give your answer in [[]] format.
\end{itemize}


\vspace{0.5em}
\textbf{\#\#\# Answer:}

\vspace{1em} % 添加间距分割两部分

%three-shot部分
\textbf{Three-shot}
\vspace{0.5em}  
\hrule % 添加水平线作为分割线  
\vspace{0.5em}  

You are an intelligent assistant that helps with various logical reasoning tasks. Below is a custom-defined rule for a specific type of logic. When responding, please ensure that your output adheres to the specified logical rules and format.

\vspace{0.5em}
\textbf{\#\#\# Instructions:}

\begin{enumerate}
    \item Identify the relevant properties and objects as specified in the rule.
    \item Apply the given logical operations or reasoning patterns.
    \item Ensure your output is formatted according to the specified notation and symbols.
\end{enumerate}

\vspace{0.5em}
\textbf{\#\#\# Logic Rule:}
\begin{itemize}[leftmargin=2em]
    \item[] \textbf{Custom Cooperation Principles}

    \begin{itemize}[leftmargin=2em]
        \item[] \textbf{C* Principle}
        \begin{enumerate}[leftmargin=2em]
            \item Speaker's Criterion: Do not let your statement be weaker in information than what your knowledge allows, unless a stronger statement conflicts with the Information Principle.
            \item Hearer's Inference:
            \begin{itemize}[left=2em]
            \item CQ1: If the speaker says $A(w)$, and $\langle s, w \rangle$ brackets the words in order of information strength with $s$ (strong) followed by $w$ (weak), $A(s)$ entails $A(w)$, then it can be inferred that $K \sim (A(s))$, meaning the speaker knows that the stronger information cannot be established.
            \item CQ2: The speaker states $A(w)$, which does not entail the content of the embedded sentence $Q$, but the content of $Q$ is entailed by the stronger information $A(s)$, and $\{s, w\}$ form a contrast set, then it can be deduced that $\sim K(Q)$, meaning the speaker does not know whether $Q$ can be established.
            \end{itemize}
        \end{enumerate}

        \item[] \textbf{C\% Principle}
        \begin{enumerate}[leftmargin=2em]
            \item Speaker's Criterion: Minimalization Criterion - Speak as little as possible, only speak to the minimum extent necessary to achieve the purpose of communication.
            \item Hearer's Inference:
            \begin{itemize}[leftmargin=2em]
                \item CI1: Assume that the relationship between the objects and time in the sentence follows the convention unless there is clear evidence to the contrary.
                \item CI2: If a certain existence or fact exactly matches the confirmed situation, it is set that this is what the sentence is saying. The Information Principle actually refers to the speaker striving to "speak as little as possible," while the hearer strives to "expand the information" until fully grasping the intention of the speech.
            \end{itemize}
        \end{enumerate}

        \item[] \textbf{C! Principle}
        \begin{enumerate}[leftmargin=2em]
            \item Speaker's Criterion: Do not use lengthy, obscure, or marked expressions without reason.
            \item Hearer's Inference: If the speaker uses a lengthy marked expression, their meaning is different from what they could have expressed with an unmarked expression, especially they should try to avoid conventional associations or derive meanings using the Information Principle.
        \end{enumerate}
    \end{itemize}

\end{itemize}

\vspace{0.5em}
\textbf{\#\#\# Question:}
\begin{itemize}[leftmargin=2em]
    \item[] In this dialogue, B’s response “She will do her best” is somewhat vague and does not directly address whether “she will be able to complete the project on time.” This response suggests that the statement “she will complete the project on time” might not be true, as “doing her best” indicates there is a risk she might not finish on time.
    \item[] Which principle does this conform to?
    \begin{itemize}[leftmargin=2em]
        \item[] A. C* Principle
        \item[] B. C\% Principle
        \item[] C. C! Principle
    \end{itemize}
    \item[] Please give your answer in the format [[A/B/C]].
\end{itemize}

\vspace{0.5em}
\textbf{\#\#\# Answer:}
\begin{itemize}[leftmargin=2em]
    \item[] [[A]]
\end{itemize}

\vspace{0.5em}
\textbf{\#\#\# Question:}
\begin{itemize}[leftmargin=2em]
    \item[] "Please open the gift box." → The gift has a box.
    \item[] Which principle does this conform to?
    \begin{itemize}[leftmargin=2em]
        \item[] A. C* Principle
        \item[] B. C\% Principle
        \item[] C. C! Principle
    \end{itemize}
    \item[] Please give your answer in the format [[A/B/C]].
\end{itemize}

\vspace{0.5em}
\textbf{\#\#\# Answer:}
\begin{itemize}[leftmargin=2em]
    \item[] [[B]]
\end{itemize}

\vspace{0.5em}
\textbf{\#\#\# Question:}
\begin{itemize}[leftmargin=2em]
    \item[] A: "Can you complete the report by the end of today?"  
    \item[] B: "I finished the report."  
    \item[] C: "After working overtime and multiple revisions, I finally got the report done."
    \item[] In this dialogue, B's response, "I finished the report," is a direct and conventional answer, indicating that B has successfully completed the report. In contrast, C's response, "After working overtime and multiple revisions, I finally got the report done," uses a lengthy and marked expression. This implies that the process of completing the report was very challenging and complex, involving additional effort and difficulties. C's response not only indicates the completion of the task but also emphasizes the hardships encountered during the process.
    \item[] C's use of a lengthy and marked expression, compared to B's concise response, provides extra information and background.
    \item[] Which principle does this conform to?
    \begin{itemize}[leftmargin=2em]
        \item[] A. C* Principle
        \item[] B. C\% Principle
        \item[] C. C! Principle
    \end{itemize}
    \item[] Please give your answer in the format [[A/B/C]].
\end{itemize}

\vspace{0.5em}
\textbf{\#\#\# Answer:}
\begin{itemize}[leftmargin=2em]
    \item[] [[C]]
\end{itemize}

\vspace{0.5em}
\textbf{\#\#\# Question:}
\begin{itemize}[leftmargin=2em]
    \item[] A: "Do you have tickets for tonight's movie?"  
    \item[] B: "I bought two tickets."  
    \item[] C: "I managed to get two tickets."
    \item[] C uses "managed to get" instead of directly saying "bought," implying that "getting the tickets was not easy and took some effort."
    \item[] Which of the following principles does this conform to?
    \begin{itemize}[leftmargin=2em]
        \item[] A. C* Principle
        \item[] B. C\% Principle
        \item[] C. C! Principle
    \end{itemize}
    \item[] Please give your answer in the format [[A/B/C]].
\end{itemize}

\vspace{0.5em}
\textbf{\#\#\# Answer:}

\end{purplebluebox}










==> prompt/operation_old.tex <==
\newtcolorbox[auto counter, number within=section]{mybox}[2][]{%
  colback=cyan!5, % Background color (light sky blue)
  colframe=cyan, % Frame color (sky blue)
  width=\textwidth, % Box width equal to page width
  sharp corners, % Sharp corners
  boxrule=0.8mm, % Border thickness
  title=\large #2, % Caption text with smaller font size
  breakable, % Supports page breaks
  fonttitle=\small, % Title font size
  fontupper=\footnotesize, % Content font size
  #1 % Additional options
}

% Example usage of the custom box with two parts (zero-shot and three-shot)
\begin{mybox}[label={mybox:example}]{Operation}
\textbf{Zero-shot}

\vspace{0.5em}  
\hrule % 添加水平线作为分割线  
\vspace{0.5em}  
You are an intelligent assistant specializing in evaluating custom operations. Below is a specific rule defined for a custom operation. Your task is to apply this rule accurately to the provided question.

\vspace{0.5em}  
\textbf{\#\#\# Instructions:}

\begin{enumerate}
    \item Carefully read and understand the definitions of the new operations in the rule.
    \item If the question does not specifically ask for it, your answer should be a number or a group of numbers.
    \item Double-check your final answer to ensure it follows the rule accurately.
\end{enumerate}

\vspace{0.5em}  
\textbf{\#\#\# Operation Rule:}

\setlength{\itemindent}{1em}
\begin{itemize}[leftmargin=2em]
    \item[] a\textyen{}b=$a^b-b^a$.
    \item[] a and b are positive integers.
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Question:}
\begin{itemize}[leftmargin=2em]
    \item[] Compute 3\textyen{}2
    \item[] Please wrap the answer in double square brackets, like this: [[]].
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Answer:}

\vspace{1em} % 添加间距分割两部分

%three-shot部分
\textbf{Three-shot}
\vspace{0.5em}  
\hrule % 添加水平线作为分割线  
\vspace{0.5em}  

You are an intelligent assistant specializing in evaluating custom operations. Below is a specific rule defined for a custom operation. Your task is to apply this rule accurately to the provided question.

\vspace{0.5em}  
\textbf{\#\#\# Instructions:}
\begin{enumerate}
    \item Carefully read and understand the definitions of the new operations in the rule.
    \item If the question does not specifically ask for it, your answer should be a number or a group of numbers.
    \item Double-check your final answer to ensure it follows the rule accurately.
\end{enumerate}

\vspace{0.5em}  
\textbf{\#\#\# Operation Rule:}
\begin{itemize}[leftmargin=2em]
    \item[] A\&B denotes the element-by-element power operation \((A \& B)_{ij} = A_{ij}^{B_{ij}}\) of matrix \(A\) and matrix \(B\).
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Question:}
\[
A =
\begin{pmatrix}
2 & 3 \\
4 & 5
\end{pmatrix}
\]
\[
B =
\begin{pmatrix}
1 & 0 \\
2 & 4
\end{pmatrix}
\]
\begin{itemize}[leftmargin=2em]
    \item[] Compute \(A \& B\).
    \item[] The answer is a matrix, write it in this form: [[((a,b),(c,d))]]
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Answer:}
\begin{itemize}[leftmargin=2em]
    \item[] [[((2,1),(16,625))]]
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Question:}
\[
A =
\begin{pmatrix}
5 & 6 \\
7 & 8
\end{pmatrix}
\]
\[
B =
\begin{pmatrix}
1 & 1 \\
3 & 2
\end{pmatrix}
\]
\begin{itemize}[leftmargin=2em]
    \item[] Compute \(A \& B\).
    \item[] The answer is a matrix, write it in this form: [[((a,b),(c,d))]]
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Answer:}
\begin{itemize}[leftmargin=2em]
    \item[] [[((5,6),(343,64))]]
\end{itemize}


\vspace{0.5em}  
\textbf{\#\#\# Question:}
\[
A =
\begin{pmatrix}
1 & 3 \\
4 & 6
\end{pmatrix}
\]
\[
B =
\begin{pmatrix}
3 & 2 \\
1 & 0
\end{pmatrix}
\]
\begin{itemize}[leftmargin=2em]
    \item[] Compute \(A \& B\).
    \item[] The answer is a matrix, write it in this form: [[((a,b),(c,d))]]
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Answer:}
\begin{itemize}[leftmargin=2em]
    \item[] [[((1,9),(4,1))]]
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Question:}
\[
A =
\begin{pmatrix}
1 & 2 \\
3 & 4
\end{pmatrix}
\]
\[
B =
\begin{pmatrix}
0 & 1 \\
2 & 3
\end{pmatrix}
\]
\begin{itemize}[leftmargin=2em]
    \item[] Compute \(A \& B\).
    \item[] The answer is a matrix, write it in this form: [[((a,b),(c,d))]]
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Answer:}

\end{mybox}


















==> prompt/puzzle_old.tex <==
\newtcolorbox[auto counter, number within=section]{redbox}[2][]{%
  colback=red!5, % Background color (very light red)
  colframe=red!50, % Frame color (pure red)
  width=\textwidth, % Box width equal to page width
  sharp corners, % Sharp corners
  boxrule=0.8mm, % Border thickness
  title=\large #2, % Caption text with smaller font size
  breakable, % Supports page breaks
  fonttitle=\small, % Title font size
  fontupper=\footnotesize, % Content font size
  #1 % Additional options
}

% Example usage of the custom box with two parts (zero-shot and three-shot)
\begin{redbox}[label={mybox:example}]{Puzzle}
\textbf{Zero-shot}

\vspace{0.5em}  
\hrule % 添加水平线作为分割线  
\vspace{0.5em}  
You are an intelligent assistant specializing in solving custom puzzle problems. Below is a specific rule defined for a custom puzzle. Your task is to apply this rule accurately to the provided question.

\vspace{0.5em}  
\textbf{\#\#\# Instructions:}

\begin{enumerate}
    \item Thoroughly understand the rule provided. If needed, break down the rule into simpler components or steps.
    \item Apply the rule carefully to address the question presented.
\item Verify your answer to ensure it aligns with the rule and the context of the puzzle. 
\end{enumerate}

\vspace{0.5em}  
\textbf{\#\#\# Puzzle Rule:}

\setlength{\itemindent}{1em}
\begin{itemize}[leftmargin=2em]
    \item[] The game gives a formula of letters, each representing a unique number (0-9).
\item[] Different letters cannot represent the same number.
\item[] The first letter of any multi-digit number cannot represent 0.
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Question:}
\begin{itemize}[leftmargin=2em]
    \item[] FORTY+TEN+TEN=SIXTY
    \item[] Answers should be given in the form: letter=number,e.g.[[A=1,B=2...]].
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Answer:}

\vspace{1em} % 添加间距分割两部分

%three-shot部分
\textbf{Three-shot}
\vspace{0.5em}  
\hrule % 添加水平线作为分割线  
\vspace{0.5em}  

You are an intelligent assistant specializing in solving custom puzzle problems. Below is a specific rule defined for a custom puzzle. Your task is to apply this rule accurately to the provided question.

\vspace{0.5em}  
\textbf{\#\#\# Instructions:}
\begin{enumerate}
    \item Thoroughly understand the rule provided. If needed, break down the rule into simpler components or steps.
    \item Apply the rule carefully to address the question presented.
    \item Verify your answer to ensure it aligns with the rule and the context of the puzzle.
\end{enumerate}

\vspace{0.5em}  
\textbf{\#\#\# Puzzle Rule:}
\begin{itemize}[leftmargin=2em]
\item[] The puzzles are played on a grid and the questions are given in the form of a matrix, consisting of X and 0.
\item[] The player needs to replace X for filling in d letters and 0 for separating words that cannot be filled in with letters.
\item[] Two lists of words are given, across and down. Across means fill in the words from left to right, and down means fill in the words from top to bottom.
\item[] During the game, many words will cross each other and share some letters.The letters that cross must match.
\item[] The question consists of a list of words and a matrix, where X denotes a grid to be filled with letters and 0 denotes a grid that does not need to be filled with letters,e.g.
\\X X X
\\0 X 0
\\0 X 0
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Question:}
across:SAD SAVE
down:ADS VASE SAVED
\begin{itemize}[leftmargin=2em]
    \item[] X X X X 0
    \item[] X 0 X 0 X
    \item[] X 0 X X X
    \item[] X 0 X 0 X
    \item[] X 0 0 0 0
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Answer:}
\begin{itemize}[leftmargin=2em]
    \item[] [[S A V E 0,A 0 A 0 A,V 0 S A D,E 0 E 0 S,D 0 0 0 0]]
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Question:}
across:CAB CUB SCUBA
down:ABS CABS CUBS

\begin{itemize}[leftmargin=2em]
    \item[] X X X 0 0 X
    \item[] X 0 0 X X X
    \item[] X 0 0 X 0 X
    \item[] X X X X X 0
    \item[] 0 0 0 X 0 0
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Answer:}
\begin{itemize}[leftmargin=2em]
    \item[] [[C A B 0 0 A,A 0 0 C U B,B 0 0 U 0 S,S C U B A 0,0 0 0 A 0 0]]
\end{itemize}


\vspace{0.5em}  
\textbf{\#\#\# Question:}
across:LOSE ROSE ROLES
down:ORE SOLE SORE
\begin{itemize}[leftmargin=2em]
    \item[] 0 0 0 X 0 0 0
    \item[] 0 0 0 X X X X
    \item[] X X X X 0 X 0
    \item[] 0 0 X 0 0 X 0
    \item[] 0 0 X X X X X
    \item[] 0 0 X 0 0 0 0
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Answer:}
\begin{itemize}[leftmargin=2em]
    \item[] [[0 0 0 O 0 0 0,0 0 0 R O S E,L O S E 0 O 0,0 0 O 0 0 L 0,0 0 R O L E S,0 0 E 0 0 0 0]]
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Question:}
across:ACT
down:CAT

\begin{itemize}[leftmargin=2em]
    \item[] X        X        X
    \item[] 0        X        0
    \item[] 0        X        0
\end{itemize}

\vspace{0.5em}  
\textbf{\#\#\# Answer:}
\end{redbox}

==> rule/test.tex <==
% \documentclass{article}
% % \usepackage[T1]{fontenc}
% % \usepackage{lmodern}
% % \usepackage{textcomp}
% % \usepackage[utf8]{inputenc}

% \usepackage{stringenc}
% \newcommand*{\uni}{}
% \DeclareRobustCommand*{\uni}[1]{%
%   \begingroup
%     \StringEncodingConvert\x{%
%       \pdfunescapehex{%
%         00%
%         \ifnum"#1<"100000 0\fi
%         \ifnum"#1<"10000 0\fi
%         \ifnum"#1<"1000 0\fi
%         \ifnum"#1<"100 0\fi
%         \ifnum"#1<"10 0\fi
%         #1%
%       }%
%     }{utf32be}{utf8}%
%     \everyeof{\noexpand}%
%     \endlinechar=-1 %
%   \edef\x{%
%     \endgroup
%     \scantokens\expandafter{%
%       \expandafter\unexpanded\expandafter{\x}%
%     }%
%   }\x
% }

% % hyperref support
% \usepackage[pdfencoding=auto]{hyperref}
% \pdfstringdefDisableCommands{%
%   \def\uni#1{\unichar{"#1}}%
% }

% \begin{document}
% \section{\uni{266A} in title}
% Symbols: \uni{a66e}, \uni{B1}, \uni{20AC}, \uni{DF}.
% \end{document}

==> self_correction/self_correction_five_figs.tex <==
\begin{figure}[htbp]
    \centering
    \subfloat[1]{
        \includegraphics[width=0.3\textwidth]{img/self_correction/operation_self_acc.pdf}
    }
    \subfloat[2]{
        \includegraphics[width=0.3\textwidth]{img/self_correction/logic_self_acc.pdf}
    }
    \subfloat[3]{
        \includegraphics[width=0.3\textwidth]{img/self_correction/cipher_self_acc.pdf}
    }
    
    \subfloat[4]{
        \includegraphics[width=0.3\textwidth]{img/self_correction/puzzle_self_acc.pdf}
    }
    \subfloat[5]{
        \includegraphics[width=0.3\textwidth]{img/self_correction/counterfactual_self_acc.pdf}
    }
    \caption{sample}
    \label{fig:five_subfigs}
\end{figure}

==> table/comparison_table.tex <==
\begin{table}[htbp]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ccccccc}
        \hline
        \multirow{2}{*}{\textbf{Benchmark}} & \multirow{2}{*}{\textbf{Domain}} & \multirow{2}{*}{\textbf{Size}} & \multicolumn{3}{c}{\textbf{Evaluation Dimensions}} & \multirow{2}{*}{\textbf{Task}} \\ 
        \cline{4-6}
        & & & \textbf{Knowledge Foundation} & \textbf{Knowledge Integration} & \textbf{Interference Control} & \\ 
        \hline
        Benchmark & Language & Large & \greencheck & \redmark & \redmark & Multiple-Choice QA \\
        KOR-Bench & Multi-domain & 1250 & \greencheck & \greencheck & \greencheck & Free-Response QA \\
       
        
    \end{tabular}
    }
    \caption{Benchmark Evaluations with Domain, Size, and Task.The "Interference Control" dimension focuses on assessing Knowledge Integration while minimizing the impact of Knowledge Foundation to ensure a clear and accurate measurement of the targeted capability. }
    \label{tab:benchmark_evaluation}
\end{table}







==> table/mixed.tex <==
\definecolor{skyblue}{RGB}{173, 216, 230}  % 天蓝色
\definecolor{lavender}{RGB}{230, 190, 255}  % 薰衣草紫

\begin{table}[h]
\centering
\resizebox{1\textwidth}{!}{%
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{Overall} & \textbf{Multi-Q} & \textbf{Multi-R} & \textbf{Multi-RQ} \\
\midrule
Claude-3.5-Sonnet & \colorbox{skyblue}{31.37} (\colorbox{lavender}{43.24}) & \colorbox{skyblue}{23.40} (\colorbox{lavender}{42.25}) & \colorbox{skyblue}{45.20}(\colorbox{lavender}{45.20}) & \colorbox{skyblue}{25.50} (\colorbox{lavender}{42.28}) \\
Qwen2.5-32B-Instruct & \textbf{23.97} (\textbf{33.96}) & \textbf{20.00} (\textbf{35.13}) & \textbf{33.40}(\textbf{33.40}) & \textbf{19.90} (\textbf{33.33}) \\
Yi-Large & \underline{22.73} (\underline{31.11}) & 14.90 (29.09) & \textbf{33.40}(\textbf{33.40}) & 19.90 (\underline{30.85}) \\
Gpt-4O & 21.80 (29.40) & 15.00 (25.39) & \underline{31.20}(\underline{31.20}) & \underline{19.20} (31.62) \\
Deepseek-V2.5 & 21.23 (31.12) & \underline{16.50} (\underline{31.88}) & 28.70(28.70) & 18.50 (32.77) \\
Mistral-Large-Instruct-2407 & 18.27 (26.31) & 14.80 (27.91) & 25.10(25.10) & 14.90 (25.92) \\
Qwen2-72B-Instruct & 17.73 (27.03) & 14.70 (28.46) & 24.60(24.60) & 13.90 (28.03) \\
Meta-Llama-3.1-70B-Instruct & 17.60 (24.71) & 14.70 (24.59) & 23.90(23.90) & 14.20 (25.63) \\
C4Ai-Command-R-08-2024 & 16.13 (23.64) & 10.40 (21.79) & 26.10(26.10) & 11.90 (23.03) \\
Qwen2.5-72B-Instruct & 13.53 (21.26) & 13.30 (25.58) & 16.00(16.00) & 11.30 (22.20) \\
Mistral-7B-Instruct-V0.3 & 9.57 (15.52) & 4.20 (13.36) & 17.70(17.70) & 6.80 (15.50) \\
C4Ai-Command-R-Plus-08-2024 & 9.53 (17.37) & 11.00 (22.94) & 9.60(9.60) & 8.00 (19.58) \\
Qwen2-7B-Instruct & 7.47 (14.03) & 7.50 (17.87) & 8.90(8.90) & 6.00 (15.33) \\
Meta-Llama-3.1-8B-Instruct & 7.00 (9.06) & 7.60 (11.32) & 8.10(8.10) & 5.30 (7.77) \\
Qwen2.5-7B-Instruct & 6.77 (12.34) & 5.40 (13.79) & 9.80(9.80) & 5.10 (13.42) \\
Yi-1.5-9B-Chat & 4.10 (9.47) & 5.30 (16.16) & 4.90(4.90) & 2.10 (7.33) \\
\bottomrule
\end{tabular}
}
\caption{Mixed Task Performance}
\label{mixed}
\end{table}

==> table/model.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{Size} & \textbf{Release Date} & \textbf{Open} & \textbf{Link} \\
\midrule
\rowcolor{blue!10} % Light blue color for the header row
\multicolumn{5}{c}{Chat Model} \\
\midrule
\href{https://example.com/gpt-40}{gpt-40} & 175B & 2024-01-15 & Yes & \href{https://example.com/gpt-40}{gpt-40} \\
\href{https://example.com/gpt-4-turbo}{gpt-4-turbo} & 150B & 2023-11-01 & Yes & \href{https://example.com/gpt-4-turbo}{gpt-4-turbo} \\
\href{https://example.com/meta-llama-3-70b-instruct}{Meta-Llama-3-70B-Instruct} & 70B & 2024-02-10 & No & \href{https://example.com/meta-llama-3-70b-instruct}{Meta-Llama-3-70B-Instruct} \\
\href{https://example.com/deepseek-v2}{deepseek-v2} & 55B & 2024-03-05 & No & \href{https://example.com/deepseek-v2}{deepseek-v2} \\
\href{https://example.com/qwen2-72b-instruct}{Qwen2-72B-Instruct} & 72B & 2024-04-20 & Yes & \href{https://example.com/qwen2-72b-instruct}{Qwen2-72B-Instruct} \\
\href{https://example.com/yi-large}{yi-large} & 50B & 2024-05-15 & No & \href{https://example.com/yi-large}{yi-large} \\
\href{https://example.com/yi-1.5-34b-chat}{Yi-1.5-34B-Chat} & 34B & 2024-06-01 & Yes & \href{https://example.com/yi-1.5-34b-chat}{Yi-1.5-34B-Chat} \\
\href{https://example.com/yi-1.5-9b-chat}{Yi-1.5-9B-Chat} & 9B & 2024-07-10 & No & \href{https://example.com/yi-1.5-9b-chat}{Yi-1.5-9B-Chat} \\
\href{https://example.com/meta-llama-3-8b-instruct}{Meta-Llama-3-8B-Instruct} & 8B & 2024-08-25 & Yes & \href{https://example.com/meta-llama-3-8b-instruct}{Meta-Llama-3-8B-Instruct} \\
\href{https://example.com/phi-3-mini-4k-instruct}{Phi-3-mini-4k-instruct} & 4k & 2024-09-15 & No & \href{https://example.com/phi-3-mini-4k-instruct}{Phi-3-mini-4k-instruct} \\
\href{https://example.com/yi-1.5-6b-chat}{Yi-1.5-6B-Chat} & 6B & 2024-10-05 & No & \href{https://example.com/yi-1.5-6b-chat}{Yi-1.5-6B-Chat} \\
\href{https://example.com/mistral-7b-instruct-v0.3}{Mistral-7B-Instruct-v0.3} & 7B & 2024-11-01 & Yes & \href{https://example.com/mistral-7b-instruct-v0.3}{Mistral-7B-Instruct-v0.3} \\
\href{https://example.com/map-neo-7b-instruct-v0.1}{MAP-Neo-7B-Instruct-v0.1} & 7B & 2024-12-01 & No & \href{https://example.com/map-neo-7b-instruct-v0.1}{MAP-Neo-7B-Instruct-v0.1} \\
\href{https://example.com/qwen2-7b-instruct}{Qwen2-7B-Instruct} & 7B & 2024-12-15 & Yes & \href{https://example.com/qwen2-7b-instruct}{Qwen2-7B-Instruct} \\
\href{https://example.com/qwen2-1.5b-instruct}{Qwen2-1.5B-Instruct} & 1.5B & 2025-01-10 & No & \href{https://example.com/qwen2-1.5b-instruct}{Qwen2-1.5B-Instruct} \\
\href{https://example.com/olmo-7b-instruct-hi}{OLMo-7B-Instruct-hí} & 7B & 2025-02-01 & No & \href{https://example.com/olmo-7b-instruct-hi}{OLMo-7B-Instruct-hí} \\
\href{https://example.com/minicpm-2b-dpo-bf16}{MiniCPM-2B-dpo-bf16} & 2B & 2025-03-01 & No & \href{https://example.com/minicpm-2b-dpo-bf16}{MiniCPM-2B-dpo-bf16} \\
\href{https://example.com/minicpm-2b-sft-bf16}{MiniCPM-2B-sft-bf16} & 2B & 2025-04-15 & No & \href{https://example.com/minicpm-2b-sft-bf16}{MiniCPM-2B-sft-bf16} \\
\href{https://example.com/qwen2-0.5b-instruct}{Qwen2-0.5B-Instruct} & 0.5B & 2025-05-10 & No & \href{https://example.com/qwen2-0.5b-instruct}{Qwen2-0.5B-Instruct} \\
\midrule
\rowcolor{green!10} % Light green color for the header row
\multicolumn{5}{c}{Base Model} \\
\midrule
\href{https://example.com/meta-llama-3-70b}{Meta-Llama-3-70B} & 70B & 2024-01-10 & No & \href{https://example.com/meta-llama-3-70b}{Meta-Llama-3-70B} \\
\href{https://example.com/qwen2-72b}{Qwen2-72B} & 72B & 2024-02-15 & Yes & \href{https://example.com/qwen2-72b}{Qwen2-72B} \\
\href{https://example.com/yi-1.5-9b}{Yi-1.5-9B} & 9B & 2024-03-05 & No & \href{https://example.com/yi-1.5-9b}{Yi-1.5-9B} \\
\href{https://example.com/qwen2-7b}{Qwen2-7B} & 7B & 2024-04-20 & Yes & \href{https://example.com/qwen2-7b}{Qwen2-7B} \\
\href{https://example.com/yi-1.5-34b}{Yi-1.5-34B} & 34B & 2024-05-15 & No & \href{https://example.com/yi-1.5-34b}{Yi-1.5-34B} \\
\href{https://example.com/meta-llama-3-8b}{Meta-Llama-3-8B} & 8B & 2024-06-01 & Yes & \href{https://example.com/meta-llama-3-8b}{Meta-Llama-3-8B} \\
\href{https://example.com/yi-1.5-6b}{Yi-1.5-6B} & 6B & 2024-07-10 & No & \href{https://example.com/yi-1.5-6b}{Yi-1.5-6B} \\
\href{https://example.com/mistral-7b-v0.3}{Mistral-7B-v0.3} & 7B & 2024-08-25 & Yes & \href{https://example.com/mistral-7b-v0.3}{Mistral-7B-v0.3} \\
\href{https://example.com/map-neo-7b}{MAP-Neo-7B} & 7B & 2024-09-15 & No & \href{https://example.com/map-neo-7b}{MAP-Neo-7B} \\
\href{https://example.com/minicpm-2b-128k}{MinicPM-2B-128k} & 2B & 2024-10-05 & No & \href{https://example.com/minicpm-2b-128k}{MinicPM-2B-128k} \\
\href{https://example.com/qwen2-1.5b}{Qwen2-1.5B} & 1.5B & 2024-11-01 & No & \href{https://example.com/qwen2-1.5b}{Qwen2-1.5B} \\
\href{https://example.com/qwen2-0.5b}{Qwen2-0.5B} & 0.5B & 2024-12-01 & No & \href{https://example.com/qwen2-0.5b}{Qwen2-0.5B} \\
\bottomrule
\end{tabular}
\caption{Model Information: Chat Models and Base Models}
\label{tab:model_info}
\end{table}


==> table/results_1121_zero_shot_cot.tex <==
\begin{table}[h!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccc}
\toprule
\textbf{Model} & \textbf{Size} & \textbf{Open} & \textbf{Overall} & \textbf{Operation} & \textbf{Logic} & \textbf{Cipher} & \textbf{Puzzle} & \textbf{Counterfactual} \\
\midrule
\href{https://platform.openai.com/docs/models/gpt-4o}{gpt-4o}\citep{openai2024gpt4o} & * & \redmark  & 55.36 & 84.40 & 50.80 & 34.00 & 16.00 & 91.60(6.40) \\ 
\href{https://huggingface.co/Qwen/Qwen2.5-32B-Instruct}{Qwen2.5-32B-Instruct}\citep{qwen2.5} & 32B & \greencheck & 55.20 & 91.20 & 59.20 & 26.80 & 8.40 & 90.40(8.00) \\ 
\href{https://huggingface.co/Qwen/Qwen2.5-72B-Instruct}{Qwen2.5-72B-Instruct}\citep{qwen2.5} & 72.7B & \greencheck & 53.12 & 84.80 & 54.80 & 31.20 & 8.40 & 86.40(10.80) \\ 
\href{https://huggingface.co/mistralai/Mistral-Large-Instruct-2407}{Mistral-Large-Instruct-2407}\citep{mistral2024} & 123B & \greencheck & 53.04 & 85.60 & 46.40 & 29.60 & 13.60 & 90.00(8.40) \\ 
\href{https://huggingface.co/deepseek-ai/DeepSeek-V2.5}{DeepSeek-V2.5}\citep{deepseekv2} & 236B & \greencheck & 52.48 & 77.20 & 55.20 & 30.80 & 10.00 & 89.20(8.00) \\ 
\href{https://huggingface.co/meta-llama/Meta-Llama-3.1-70B-Instruct}{Meta-Llama-3.1-70B-Instruct}\citep{dubey2024llama} & 70B & \greencheck & 50.64 & 86.80 & 46.00 & 21.20 & 8.80 & 90.40(7.20) \\ 
\href{https://platform.lingyiwanwu.com/}{yi-large}\citep{} & * & \redmark  & 49.52 & 82.80 & 46.80 & 20.00 & 11.60 & 86.40(10.80) \\ 
\href{https://huggingface.co/Qwen/Qwen2-72B-Instruct}{Qwen2-72B-Instruct}\citep{qwen2} & 72.71B & \greencheck & 49.20 & 79.60 & 47.60 & 19.20 & 8.80 & 90.80(7.20) \\ 
\href{https://huggingface.co/Qwen/Qwen2.5-7B-Instruct}{Qwen2.5-7B-Instruct}\citep{qwen2.5} & 7.61B & \greencheck & 44.96 & 80.00 & 41.20 & 13.20 & 4.40 & 86.00(8.80) \\ 
\href{https://www.anthropic.com/news/claude-3-5-sonnet}{claude-3-5-sonnet-20240620}\citep{claude35addendum} & * & \redmark  & 44.24 & 58.40 & 48.00 & 16.40 & 7.20 & 91.20(6.00) \\ 
\href{https://huggingface.co/01-ai/Yi-1.5-9B-Chat}{Yi-1.5-9B-Chat}\citep{ai2024yiopenfoundationmodels} & 9B & \greencheck & 39.20 & 79.60 & 24.80 & 8.80 & 3.20 & 79.60(9.60) \\ 
\href{https://huggingface.co/CohereForAI/c4ai-command-r-plus-08-2024}{c4ai-command-r-plus-08-2024}\citep{} & 104B & \greencheck & 37.92 & 47.60 & 39.60 & 8.40 & 2.80 & 91.20(5.60) \\ 
\href{https://huggingface.co/meta-llama/Meta-Llama-3.1-8B-Instruct}{Meta-Llama-3.1-8B-Instruct}\citep{dubey2024llama} & 8B & \greencheck & 35.84 & 59.60 & 26.40 & 9.20 & 3.60 & 80.40(6.80) \\ 
\href{https://huggingface.co/CohereForAI/c4ai-command-r-08-2024}{c4ai-command-r-08-2024}\citep{} & 32B & \greencheck & 34.56 & 45.60 & 30.80 & 6.00 & 3.20 & 87.20(7.60) \\ 
\href{https://huggingface.co/Qwen/Qwen2-7B-Instruct}{Qwen2-7B-Instruct}\citep{qwen2} & 7.07B & \greencheck & 31.92 & 42.40 & 27.20 & 6.80 & 2.00 & 81.20(7.60) \\ 
\href{https://huggingface.co/mistralai/Mistral-7B-v0.3}{Mistral-7B-Instruct-v0.3}\citep{jiang2023mistral7b} & 7B & \greencheck & 25.52 & 24.00 & 16.80 & 5.60 & 2.00 & 79.20(11.20) \\ 
\bottomrule
\end{tabular}
}
\caption{Models Performance on KOR-Bench *Note: Values in parentheses represent the proportion of responses where the model provided the real-world answers in the counterfactual setting.*}
\label{zero_cot}
\end{table}


==> table/rule_length.tex <==
\begin{table}[h]
    \centering
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{lcccc}
        \toprule
        \textbf{Category} & \multicolumn{2}{c}{\textbf{Text}} & \multicolumn{2}{c}{\textbf{Token}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5}
        & Mean & Std. Dev. & Mean & Std. Dev. \\
        \midrule
        Operation & 51.28 & 43.50 & 21.60 & 12.07 \\
        Logic & 1549.12 & 667.39 & 426.56 & 145.97 \\
        Cipher & 2441.12 & 1121.88 & 678.56 & 409.60 \\
        Puzzle & 473.16 & 185.09 & 108.16 & 43.37 \\
        Counterfactual & 4572.56 & 1886.30 & 942.20 & 403.87 \\
        \bottomrule
    \end{tabular}
    }
    \caption{Rule Length Statistics for Each Category. This table shows the mean and standard deviation of rule lengths across different categories, including additional statistics.}
    \label{rule_length_statistics}
\end{table}

==> table/rule_statistic.tex <==
\begin{wraptable}{r}{0.5\textwidth}
\setlength{\intextsep}{0pt}
\centering
\renewcommand{\arraystretch}{1.5} % Increase row height
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{l|l|l|c}
\hline
\textbf{Category} & \textbf{Subcategory} & \textbf{Description} & \textbf{Rule Count} \\
\hline
\multirow{8}{*}{\textbf{Operation}} 
& \multirow{2}{*}{Basic Level} & Elementary arithmetic & 6 \\
& & Power and square root & 2 \\
\cline{2-4}
& \multirow{4}{*}{Advanced Level} & Exponential and logarithmic & 4 \\
& & Operation on complex numbers & 2 \\
& & Derivative & 2 \\
& & Operation on sets & 1 \\
\cline{2-4}
& \multirow{2}{*}{Challenging Level} & Calculus & 4 \\
& & Operation on matrices & 3 \\
\hline
\multirow{6}{*}{\textbf{Logic}} 
& \multirow{4}{*}{Formal Logic} & Propositional Logic & 5 \\
& & Predicate Logic & 5 \\
& & Modal Logic & 5 \\
& & Inductive Logic & 5 \\
\cline{2-4}
& \multirow{1}{*}{Informal Logic} 
& Informal Logic & 5 \\
\hline
\multirow{8}{*}{\textbf{Cipher}} 
& \multirow{4}{*}{Classical Cryptography} & Monoalphabetic Ciphers & 5 \\
& & Polyalphabetic Ciphers & 5 \\
& & Polygraphic Ciphers & 5 \\
& & Transposition Ciphers & 5 \\
\cline{2-4}
& \multirow{3}{*}{Modern Cryptography} & Symmetric Ciphers & 2 \\
& & Asymmetric Ciphers & 2 \\
& & Hash Function Ciphers & 1 \\
\hline
\multirow{6}{*}{\textbf{Puzzle}} 
& \multirow{3}{*}{Verbal} & Verbal only  & 6  \\
& & Verbal \& Mathematical & 1\\
& & Verbal \& Spatial & 2\\
\cline{2-4}
& \multirow{2}{*}{Mathematical} & Mathematical only & 2 \\
& & Mathematical \& Spatial & 11\\
\cline{2-4}
& \multirow{1}{*}{Spatial} & Spatial only & 3\\
\hline
\multirow{1}{*}{\textbf{Counterfactual}} 
& & & 25 \\
\hline
\end{tabular}
}
\caption{Statistical Overview of Rule Distribution Across Categories}
\label{rule_statistic}
\end{wraptable}




